Causal Process Mining from Relational Databases with Domain Knowledge

The plethora of algorithms in the research field of process mining builds on directly-follows relations. Even though various improvements have been made in the last decade, there are serious weaknesses of these relationships. Once events associated with different objects that relate with a cardinality of 1:N and N:M to each other, techniques based on directly-follows relations produce spurious relations, self-loops, and back-jumps. This is due to the fact that event sequence as described in classical event logs differs from event causation. In this paper, we address the research problem of representing the causal structure of process-related event data. To this end, we develop a new approach called Causal Process Mining. This approach renounces the use of flat event logs and considers relational databases of event data as an input. More specifically, we transform the relational data structures based on the Causal Process Template into what we call Causal Event Graph. We evaluate our approach and compare its outputs with techniques based on directly-follows relations in a case study with an European food production company. Our results demonstrate the benefits for enriching process mining with additional knowledge from the domain.

==> sections/30_approach/32_preliminaries.tex <==
\subsection{Preliminaries}
\label{subsec:preliminaries}
\noindent 
%Our approach to \gls{cpm} builds on the idea to first identify the causal relationships of the observed cases before we create different aggregations of the observed cases and perform analysis operations. 

Before we present our approach to \gls{cpm}, we introduce in the following necessary preliminaries.

%We first revisit the concepts of \emph{\gls{pes}} as presented in~\cite{DBLP:journals/is/Armas-Cervantes16} based on~\cite{nielsen1981petri}. 

\begin{definition}[\acrlong{pes} {\citep{DBLP:journals/is/Armas-Cervantes16}}]
\label{def:pes}
A tuple $\mathbb{P} = \langle E, \leq, \#, \lambda \rangle$ is a labeled \acrfull{pes}, where $E$ is a set of events, $\leq$ (causality relation) is a partial order on $E$, $\#$ (conflict relation) is irreflexive, symmetric and hereditary with respect to $\leq$, namely if $e \# e' \land e' \leq e''$ then $e \# e''$ for all $e,e',e'' \in E$, and $\lambda : E \to \Lambda$ is a labeling function.
\end{definition}

According to the definition, a \gls{pes} defines the relation of causality and conflict \commentKR{We do not really have a conflict. It is a decision. Maybe another term can be used. } over events. \Cref{fig:pes_example} illustrates a \gls{pes} over the events of a simplified order-to-cash process, where solid arrows represent causality and dotted lines represent conflicts. In the process, an order $a$, causes a shipment of the item to the customer $c$ or a direct pickup $p$ by the customer. Both the shipment and the pickup generate an invoice $f$ for the customer.  
\begin{figure}[h]
    \centering
    \tikzset{>=latex}
    \begin{tikzpicture}[sibling distance=2cm, above=1cm, edge from parent/.style={draw,-latex}]
        \node {a}
        child {node (c) {c}
        child {node (f) {f} } }
        child {node (p) {p} };            
        \draw[dotted,thick] (c) -- (p);
        \draw[->] (p) -> (f);
    \end{tikzpicture}
    \caption{Example of a \gls{pes}. Solid arrows represent causality and dotted line represents conflict.}
    \label{fig:pes_example}
\end{figure}

As defined in~\Cref{def:pes}, a \gls{pes} models event types of a process, the causal relation between them, and possible decisions, e.g., picking or purchasing of an item (cf. \Cref{fig:pes_example}).  

\commentKR{@kate include examples for Definition 2 and 3}
%Furthermore, we define the following accompanying functions and concepts.
\begin{definition}[Preset and Postset Nodes] 
For a set of events $E$ and a relation $R\subseteq E \times E$, we define for an $e \in E$ the preset of nodes $\pre{e} = \{ x~|~(x,e)\in R \}$ as well as the postset of nodes $\post{e} = \{x~|~(e,x)\in R\}$.
\end{definition}
%
\begin{definition}[Event Type, Identifier and Time] 
\label{def:event_type}
Given $E$ is a set of events and $ET$ is a set of event types, we define $\tau : E \to ET$ as the function that returns the type of an event. 
We define $e^\tau=\tau(e)$. 
Furthermore, we define $\mathrm{id} : E \to I$ as an index function and $\mathrm{t}: E \to \mathbb{R}$ as a time function. 
\end{definition}
%
% \begin{definition}[Event Property] 
% \label{def:event_properties}
% For a set of events $E$ we define for an $e \in E$ and a label $\lambda \in \Lambda$ a function $\mathrm{prop} : E \times \Lambda \to \mathbb{P}$ that returns a property value for an event.\todoPW{Function that returns the event duration?}
% \end{definition}

%Finally, we define the following accompanying function to get additional event properties that are stored in the source relational \gls{db}, e.g., the duration in \Cref{fig:ceg_construction_er}.

After defining the preliminaries, the \Cref{subsec:graph-construction} discusses our approach for \gls{cpm}, called the \emph{Noreja Approach}, in detail.


==> sections/old-10_introduction.tex <==

\section{Introduction}
\label{sec:introduction}
\noindent 
Ever since its first introduction in the 1990s and the fundamental works associated with Wil van der Aalst, \gls{pm} has been established as a bridge between Data Science and Process Science with the intention to lift \gls{bpm} into the data-driven era. The movement was given a decisive boost in 2011 when more than 70 of the world's leading \gls{bpm} researchers published a manifesto \citep{van2011process} with a joint declaration on the fundamentals of \gls{dfg}. Subsequently, the strong impact of the manifesto and its key assumptions led to the development of various \gls{dfg} approaches such as the inductive miner \citep{leemans2018scalable}, the evolutionary tree miner \citep{buijs2014quality}, or the split miner \citep{augusto2019split} which all centered around the use of flat event logs with its rigid structure regarding case id, activities, and timestamps. The algorithms themselves reached a high degree of maturity and differ in their balance between fitness, simplicity, generalization, and precision in order to better cope with different event log characteristics or use cases \citep{DBLP:books/sp/Aalst16}. 

In this regard, the \gls{dfg} domain developed a tendency for path-dependent behavior and representational bias \citep{Aalst2011OnTR} that circled around the utilization of event logs and \glspl{dfg}, which limited the possibilities to analyze process data more holistically from multiple perspectives by keeping the causal references and object-relations of the underlying source data. Therefore, we argue that it is necessary to provide alternatives to the classic event log based approaches to make \gls{pm} ready for the next evolutionary stage in the era of \textit{Big Data} and the application in an organizational context. Recently, a new strain of \gls{pm} approaches around the terms object-centric \gls{pm} \citep{DBLP:conf/sefm/Aalst19, DBLP:conf/caise/LiMCA18}, artifact-related \gls{pm} \citep{DBLP:journals/tsc/LuNWF15}, or the event log generation from relational \glspl{db} \citep{DBLP:journals/kais/MurillasRA20, 10.1007/978-3-030-46633-6_2, ANDREWS2020113265} has emerged that starts to acknowledge this problem.

In this study, we want to redirect the focus of attention to the actual needs of organizations that mostly store their data in systems like ERP, SCM, PLM, CRM, or data warehouses with relational data structures (with star, snowflake, or arbitrary data schemas) since they rely on the causal relationships that the data internalize for use-case specific (data-centric) analysis. In the case companies decide to apply classical \gls{pm} approaches to analyze their processes (process-centric), they often find themselves in the challenging situation of extracting and enriching event logs out of those systems. This is especially challenging when several source systems are involved and new data objects need to be added regularly. However, this requires not only expert knowledge in the area of effective event logs creation but also the ex-ante definition of case id and activities for the flattened event log. Afterward, the resulting process representation often has weaknesses, such as spurious relationships, self-loops, or misleading aggregation levels which can lead the analyst to false conclusions \citep{Aalst2011OnTR}. This puts organizations in a paradoxical situation because the causality they take for granted for data-centric analysis is simply given up for process-centric analysis. With this study, we want to face this disparity by developing a solution for organizations to leverage the causal knowledge existing in relational data structures for process-centric analyses without sacrificing multi-dimensionality. In fact, we identified this problem as a decisive impediment to a higher \gls{pm} adaptation in the industry, especially for small- and medium-sized companies.

In this paper, we present a new approach named {\em \gls{cpm}}. This approach renounces the use of flattened event logs. Rather, it transforms the relational data structures, based on the \gls{cpt}, into what we call {\em \glspl{ceg}} and \emph{\glspl{aceg}} that are then stores inside a graph \gls{db}. \gls{cpm} exploits these structures and offers multiple operations to investigate process levels from various perspectives and at different levels of aggregation. Moreover, we evaluate \gls{cpm} and compare its outputs with techniques based on directly-follows relations in a case study with an Austrian food production company. Our results demonstrate that directly-follows miners produce heaps of spurious relationships which stem from a lack of knowledge of the underlying causal structures.
 
The rest of the paper is structured as follows. Section~\ref{sec:background} illustrates the fundamental challenges and disadvantages of \gls{dfg} by making use of a simple production scenario example. Moreover, we derive requirements in order to fully address those disadvantages. Afterward, Section~\ref{sec:approach} presents our approach of \gls{cpm} from an algorithmic perspective. Thereby, we illustrate how our approach implements cardinality, causality, and process instance aggregation. Section~\ref{sec:evaluation} conducts an evaluation between \gls{cpm} and the output produced by miners that build on directly-follows relations. Then, we discuss the implications of the evaluation results in Section~\ref{sec:discussion} before we conclude the paper in Section~\ref{sec:conclusion} with an outlook on future research.

%\\gls{pm} research over the last decade has spent considerable efforts on improving algorithms for automatic process discovery. Beside the advancements of recent algorithms such as the inductive miner~\cite{leemans2018scalable}, the evolutionary tree miner~\cite{buijs2014quality}, or the split miner~\cite{augusto2019split}, it remains a challenge to trade off accuracy and complexity of the discovered process models~\cite{augusto2018automated}. Recent miners perform well in achieving high precision and recall, but often at the price of producing so-called Spaghetti models, models that are overly complex.

%\\gls{pm} tools provide support for process analysts to handle the complexity of Spaghetti models by the help of various filtering features. The idea is to interactively zoom in on detailed behaviour that is interesting for the analyst and zoom out where context has to be understood~\cite{van2012process,vidgof2020cherry}. It is a problem, however, that the complexity presented to the analyst often goes unquestioned. van der Aalst brings in a verdict of not guilty for the benefit of \gls{pm} techniques when he states that the ``spaghetti-like structures are not caused by the discovery algorithm but by the variability of the process''~\cite{van2012process}. The scientific presumption of innocence applies, but a deeper investigation of the problem is warranted. Notably, \gls{pm} research has largely neglected the opportunity to reduce complexity by integrating causal knowledge that a process analyst can explicate or that is implicitly captured in database schemas. 

%\In this paper, we address the Spaghetti model problem by developing a new process miner technique that builds on knowledge of causality. Our starting point is the observation that causal dependencies can never be fully uncovered from the data alone. We illustrate the problem with simple examples and discuss our observation in relation to the three-level causal hierarchy by Pearl~\cite{pearl2019seven}. Our key idea to overcome this fundamental problem is to enrich observations of event sequences with knowledge of causality. To this end, we extend notions of prime and asymmetric event structures~\cite{DBLP:journals/is/Armas-Cervantes16}. Our causal miner exploits these structures and offers various operations to investigate process levels from various perspectives and at different levels of aggregation. We have implemented the causal miner and compare its output with techniques based on directly-follows relations in a case study with an Austrian food production company. Our results demonstrate that directly-follows miners produce heaps of spurious arcs which stem from a lack of knowledge of the underlying causal structures.

%\The rest of the paper is structured as follows. Section~\ref{back} presents the simple example of a production scenario, by which we illustrate the fundamental problem of \gls{pm} based on directly-follows relations. Section~\ref{approach} presents our causal miner. We extend the notions of prime and asymmetric event structures and devise operations upon them for analyzing the event log data. Section~\ref{eval} presents the evaluation of our causal miner in comparison with the output produced by miners that build on directly-follows relations. We discuss the implications of the evaluation results. Finally, Section~\ref{outro} concludes the paper with an outlook on future research.
